Exploring Dataset-Scale Indicators of Data Quality

Modern computer vision foundation models are trained on massive amounts of data, incurring large economic and environmental costs. Recent research has suggested that improving data quality can significantly reduce the need for data quantity. But what constitutes data quality in computer vision? We posit that the quality of a given dataset can be decomposed into distinct sample-level and dataset-level constituents, and that the former have been more extensively studied than the latter. We ablate the effects of two important dataset-level constituents: label set design, and class balance. By monitoring these constituents using key indicators we provide, researchers and practitioners can better anticipate model performance, measured in terms of its accuracy and robustness to distribution shifts.

==> Plots/label-set-size-002.tex <==
% This file was created with tikzplotlib v0.10.1.

\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray128}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{blue204}{RGB}{200,200,250}
\definecolor{blue128}{RGB}{100,100,190}
\definecolor{blue90}{RGB}{60,60,160}
\definecolor{red204}{RGB}{250,200,200}
\definecolor{red170}{RGB}{220,160,160}
\definecolor{red128}{RGB}{190,100,100}
\definecolor{red90}{RGB}{160,60,60}
\definecolor{red60}{RGB}{120,45,45}
\definecolor{green204}{RGB}{200,250,200}
\definecolor{green170}{RGB}{160,220,160}
\definecolor{green128}{RGB}{100,190,100}
\definecolor{green90}{RGB}{60,160,60}
\definecolor{green60}{RGB}{45,120,45}
\definecolor{green40}{RGB}{30,90,30}


\def\discon{$\wr\!\!\!\wr$}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0,1)},
  anchor=north west,
  draw=lightgray204
},
xmin=83, xmax=100,
ymin=39, ymax=75,
tick align=outside,
tick pos=left,
x grid style={lightgray204},
ylabel={IN100 Avg. Rob.},
xmajorgrids,
% xtick style={color=black},
y grid style={lightgray204},
xlabel={IN100 Val. Acc.},
ymajorgrids,
% ytick style={color=black},
% xlabel style={font=\normalsize},
% ylabel style={font=\normalsize},
% width=16cm,
% height=9cm,
% xtick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0}, %edit for number for x-labels
% ytick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
% xticklabels={$1/16\times$, $1/8\times$, $1/4\times$, $1\times$, $2\times$, $5\times$, $10\times$, $20\times$, $1000\times$, $10000\times$},
% extra x ticks = {7.5},
% extra x tick style  = {grid=none, xticklabel style={yshift=3.5mm, inner sep=.5pt}},
% extra x tick labels = {\discon},
% ]
]
\addplot [only marks, mark=square*, mark size=3.0, draw=black, mark options={fill=black}]
table{
    x y
    85.3 40.6
};
\addlegendentry{Baseline}

%resnetv2_50.a1h_in1k
\addplot [only marks, mark=*, mark size=6.0, draw=black, mark options={fill=green204}]
table{
    x y
    95.2 52.2 
};
\addlegendentry{H-Scaling}

%resnetv2_50x1_bit.goog_in21k_ft_in1k
\addplot [only marks, mark=*, mark size=8.0, draw=black, mark options={fill=green170}, forget plot]
table{
    x y
    95.8 59.0
};

%vit_base_patch16_224.augreg2_in21k_ft_in1k
\addplot [only marks, mark=*, mark size=8.0, draw=black, mark options={fill=green128}, forget plot]
table{
    x y
    97.1 66.8
};

%resnet26.bt_in1k
\addplot [only marks, mark=*, mark size=6.0, draw=black, mark options={fill=green90}, forget plot]
table{
    x y
    93.2 46.4
};

%efficientnet_b4.ra2_in1k
\addplot [only marks, mark=*, mark size=6.0, draw=black, mark options={fill=green60}, forget plot]
table{
    x y
    96.8 64.1
};

%gcvit_tiny.in1k
\addplot [only marks, mark=*, mark size=6.0, draw=black, mark options={fill=green40}, forget plot]
table{
    x y
    96.7 61.1
};


\addplot [only marks, mark=square*, mark size=6.0, draw=black, mark options={fill=red128}]
table{
    x y
    91.1 52.4
};
\addlegendentry{Fine-tuning}
\addplot [only marks, mark=square*, mark size=8.0, draw=black, mark options={fill=red90}, forget plot]
table{
    x y
    92.4 49.8
};
\addplot [only marks, mark=square*, mark size=8.0, draw=black, mark options={fill=red60}, forget plot]
table{
    x y
    88.6 50.1
};

\addlegendimage{empty legend}
\addlegendentry{(Larger points -> more data)}

\end{axis}


\end{tikzpicture}


==> Plots/meta-overfitting-001.tex <==
% This file was created with tikzplotlib v0.10.1.

\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
%\definecolor{blue}{RGB}{0,0,128}

\def\discon{$\wr\!\!\!\wr$}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.52,0.18)},
  anchor=north west,
  draw=lightgray204
},
xmin=0.6, xmax=.95,
ymin=0.35, ymax=0.6,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
ylabel={IN100 Avg. Rob.},
xmajorgrids,
% xtick style={color=black},
y grid style={darkgray176},
xlabel={IN100 Val. Acc.},
ymajorgrids,
% ytick style={color=black},
% xlabel style={font=\normalsize},
% ylabel style={font=\normalsize},
% width=16cm,
% height=9cm,
% xtick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0}, %edit for number for x-labels
% ytick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
% xticklabels={$1/16\times$, $1/8\times$, $1/4\times$, $1\times$, $2\times$, $5\times$, $10\times$, $20\times$, $1000\times$, $10000\times$},
% extra x ticks = {7.5},
% extra x tick style  = {grid=none, xticklabel style={yshift=3.5mm, inner sep=.5pt}},
% extra x tick labels = {\discon},
% ]
]
\addplot [only marks, mark=*, mark size=3.0, draw=green, mark options={fill=green}]
table{
    x y
    0.853 0.406
};
\addlegendentry{ImageNet}

\addplot [only marks, mark=*, mark size=4.5, draw=green, mark options={fill=green}, forget plot]
table{
    x y
    0.883 0.457 
};
\addplot [only marks, mark=*, mark size=6.0, draw=green, mark options={fill=green}, forget plot]
table{
    x y
    0.907 0.468 
};

\addplot [only marks, mark=triangle*, mark size=3.0, draw=blue, mark options={fill=blue}]
table{
    x y
    0.824 0.429
};
\addlegendentry{OpenImages + ImageNet (CB)}
\addplot [only marks, mark=triangle*, mark size=4.5, draw=blue, mark options={fill=blue}, forget plot]
table{
    x y
    0.858 0.477
};
\addplot [only marks, mark=triangle*, mark size=6.0, draw=blue, mark options={fill=blue}, forget plot]
table{
    x y
    0.877 0.557
};
\addplot [only marks, mark=square*, mark size=3.0, draw=red, mark options={fill=red}]
table{
    x y
    0.677 0.372
};
\addlegendentry{OpenImages}
\addplot [only marks, mark=square*, mark size=4.5, draw=red, mark options={fill=red}, forget plot]
table{
    x y
    0.644 0.370
};
\addplot [only marks, mark=square*, mark size=6.0, draw=red, mark options={fill=red}, forget plot]
table{
    x y
    0.733 0.466
};

\addlegendimage{empty legend}
\addlegendentry{(Larger points -> more data)}

\end{axis}


\end{tikzpicture}

